Confidence Calibration for Recommender Systems and Its Applications

Despite the importance of having a measure of confidence in recommendation results, it has been surprisingly overlooked in the literature compared to the accuracy of the recommendation. In this dissertation, I propose a model calibration framework for recommender systems for estimating accurate confidence in recommendation results based on the learned ranking scores. Moreover, I subsequently introduce two real-world applications of confidence on recommendations: (1) Training a small student model by treating the confidence of a big teacher model as additional learning guidance, (2) Adjusting the number of presented items based on the expected user utility estimated with calibrated probability.

==> table/6EXztable.tex <==
\begin{sidewaystable}[ph!] %\begin{table*}[ht]
 \caption{Average user utility of recommendations produced by compared methods when they are optimized for each target utility measure. \textit{Improv.} denotes the improvement of PerK over MtCut. The numbers in boldface denote the best result in each setting. *We conduct the paired t-test with a 0.05 level and every \textit{Improv.} is statistically significant.}
  \resizebox{\textwidth}{!}{% 
  \begin{tabular}{cl | cccc | cccc | cccc | cccc}
    \toprule 
     Base & \multirow{2}{*}{Method} & \multicolumn{4}{c|}{MovieLens 10M} & \multicolumn{4}{c|}{CiteULike} & \multicolumn{4}{c|}{MovieLens 25M} & \multicolumn{4}{c}{Amazon Books}\\
     Model & & NDCG & PDCG & F1 & TP &NDCG & PDCG & F1 & TP & NDCG & PDCG & F1 & TP & NDCG & PDCG & F1 & TP \\
    \toprule
    % BPR
     & Oracle &0.6190 & 0.6702  & 0.3152 & 0.7078 & 0.3020 & -0.3677  & 0.1806 & 0.3940 & 0.5961 & 0.6089  & 0.2883 & 0.6812 & 0.1895 & -0.7438  & 0.1133 & 0.2643 \\
     \cmidrule{2-18}
     & Top-1 & 0.4549 & -0.0902 & 0.0546 & 0.4549 & 0.1837 & -0.6326  & 0.0338 & 0.1837 & 0.4392 & -0.1216 & 0.0492 & 0.4392 & 0.0961 & -0.8078  & 0.0216 & 0.0961 \\
     & Top-5  &0.3925 & -0.6428 & 0.1541 & 0.3751 & 0.1489 & -2.0787  & 0.0842 & 0.1401 & 0.3729 & -0.7561 & 0.1357 & 0.3547 & 0.0786 & -2.4938  & 0.0507 & 0.0741 \\
     & Top-10  &0.3725 & -1.3715 & 0.1984 & 0.3584 & 0.1495 & -3.3650  & 0.1024 & 0.1483 & 0.3496 & -1.5372 & 0.1757 & 0.3328 & 0.0828 & -3.9401  & 0.0582 & 0.0852 \\
     & Top-20 & 0.3734 & -2.8434 & 0.2228 & 0.3849 & 0.1668 & -5.4853  & 0.1108 & 0.1907 & 0.3460 & -3.0494 & 0.2013 & 0.3510 & 0.0955 & -6.2660  & 0.0584 & 0.1155 \\
     BPR & Top-50 & 0.4057 & -7.1636 & 0.2117 & 0.4841 & 0.2021 & -10.8747 & 0.0930 & 0.2834 & 0.3740 & -7.3813 & 0.1983 & 0.4421 & 0.1203 & -11.8590 & 0.0496 & 0.1826 \\
    \cmidrule{2-18}
     & Rand & 0.3872 & -3.6387 & 0.2046 & 0.4144 & 0.1738 & -6.2622  & 0.1003 & 0.2058 & 0.3611 & -3.8266 & 0.1865 & 0.3801 & 0.0998 & -7.1022  & 0.0535 & 0.1284 \\
     & Val-$k$ & 0.4562 & -0.0640 & 0.2270 & 0.4906 & 0.1922 & -0.6162  & 0.1061 & 0.2266 & 0.4368 & -0.0532 & 0.2052 & 0.4347 & 0.1093 & -0.8378  & 0.0563 & 0.1362 \\
    \cmidrule{2-18}
     & AttnCut & 0.4604 & -0.0702 & 0.2371 & 0.4969 & 0.2024 & -0.6142  & 0.1063 & 0.2835 & 0.4392 & -0.1214 & 0.2087 & 0.4392 & 0.1203 & -0.8078  & 0.0566 & 0.1826 \\
     & MtCut & 0.4621 & -0.0167 & 0.2383 & 0.5037 & 0.2034 & -0.6022  & 0.1071 & 0.2838 & 0.4413 & -0.0616 & 0.2140 & 0.4639 & 0.1212 & -0.8078  & 0.0568 & 0.1826 \\
     \cmidrule{2-18}
     & PerK & \textbf{0.4901} & \textbf{0.2087}  & \textbf{0.2538} & \textbf{0.5711} & \textbf{0.2159} & \textbf{-0.4971}  & \textbf{0.1117} & \textbf{0.2993} & \textbf{0.4687} & \textbf{0.1876}  & \textbf{0.2300} & \textbf{0.5401} & \textbf{0.1261} & \textbf{-0.7952}  & \textbf{0.0619} & \textbf{0.1894} \\
     & \textit{Improv.} & 6.06\%* &   -      & 6.50\%* & 13.38\%* & 6.15\%* &   -       & 4.30\%* & 5.46\%* & 6.21\%* &    -     & 7.48\%* & 16.43\%* & 4.04\%* &   -       & 8.98\%* & 3.72\%* \\
    \toprule
    % NCF
     & Oracle & 0.5760 & 0.4792  & 0.2896 & 0.6688  & 0.2813 & -0.4076  & 0.1685 & 0.3690 & 0.5310 & 0.3544  & 0.2513 & 0.6157  & 0.1444 & -0.8246  & 0.0885 & 0.2076 \\
     \cmidrule{2-18}
     & Top-1  & 0.4081 & -0.1839 & 0.0474 & 0.4081  & 0.1700 & -0.6601  & 0.0304 & 0.1700 & 0.3761 & -0.2479 & 0.0393 & 0.3761  & 0.0666 & -0.8668  & 0.0150 & 0.0666 \\
     & Top-5  & 0.3521 & -0.8801 & 0.1350 & 0.3368  & 0.1403 & -2.1273  & 0.0786 & 0.1330 & 0.3206 & -1.0628 & 0.1117 & 0.3055  & 0.0563 & -2.6231  & 0.0370 & 0.0537 \\
     & Top-10  & 0.3360 & -1.6822 & 0.1764 & 0.3251  & 0.1384 & -3.4438  & 0.0942 & 0.1368 & 0.3011 & -1.9434 & 0.1474 & 0.2873  & 0.0606 & -4.1048  & 0.0434 & 0.0638 \\
     & Top-20  & 0.3397 & -3.2150 & 0.2023 & 0.3545  & 0.1529 & -5.5941  & 0.1015 & 0.1733 & 0.2980 & -3.5640 & 0.1721 & 0.3033  & 0.0712 & -6.4683  & 0.0443 & 0.0888 \\
     NCF & Top-50  & 0.3721 & -7.6021 & 0.1966 & 0.4525  & 0.1866 & -11.0026 & 0.0870 & 0.2618 & 0.3237 & -8.0277 & 0.1744 & 0.3870  & 0.0916 & -12.1148 & 0.0384 & 0.1437 \\
    \cmidrule{2-18}
     & Rand  & 0.3527 & -3.9939 & 0.1866 & 0.3821  & 0.1609 & -6.4157  & 0.0910 & 0.1884 & 0.3102 & -4.3422 & 0.1603 & 0.3298  & 0.0749 & -7.3212  & 0.0407 & 0.0987 \\
     & Val-$k$  & 0.4123 & -0.1030  & 0.2071 & 0.4554  & 0.1794 & -0.5801  & 0.0989 & 0.2101 & 0.3769 & -0.5071 & 0.1729 & 0.3842  & 0.0791 & -0.8935  & 0.0422 & 0.1018 \\
    \cmidrule{2-18}
     & AttnCut  & 0.4154 & -0.0839 & 0.2068 & 0.4612  & 0.1812 & -0.5527  & 0.0991 & 0.2619 & 0.3762 & -0.1166 & 0.1755 & 0.3994  & 0.0918 & -0.8668  & 0.0437 & 0.1438 \\
     & MtCut  & 0.4195 & 0.0805 & 0.2153 & 0.4798  & 0.1891 & -0.5499  & 0.1006 & 0.2627 & 0.3798 & -0.0142 & 0.1837 & 0.4079  & 0.0923 & -0.8667  & 0.0441 & 0.1441 \\
     \cmidrule{2-18}
     & PerK  & \textbf{0.4482} & \textbf{0.0928}  & \textbf{0.2293} & \textbf{0.5335}  & \textbf{0.2061} & \textbf{-0.5177}  & \textbf{0.1080} & \textbf{0.2764} & \textbf{0.4056} & \textbf{0.0047}  & \textbf{0.1960} & \textbf{0.4742}  & \textbf{0.0982} & \textbf{-0.8646}  & \textbf{0.0468} & \textbf{0.1553} \\
     & \textit{Improv.} & 6.84\%* &   -      & 6.50\%* & 11.19\%* & 8.99\%* &   -       & 7.36\%* & 5.22\%* & 6.79\%* &   -      & 6.70\%* & 16.25\%* & 6.39\%* &     -     & 6.12\%* & 7.77\%*\\
    \toprule
    % LightGCN
     & Oracle & 0.6249 & 0.7459  & 0.3094 & 0.7051  & 0.3471 & -0.2352  & 0.2104 & 0.4400 & 0.5893 & 0.4840  & 0.2864 & 0.6772 & 0.1782 & -0.7571  & 0.1061 & 0.2454 \\
     \cmidrule{2-18}
     & Top-1  & 0.4749 & -0.0502 & 0.0565 & 0.4749  & 0.2182 & -0.5636  & 0.0420 & 0.2182 & 0.4236 & -0.1527 & 0.0490 & 0.4236 & 0.0919 & -0.8162  & 0.0213 & 0.0919 \\
     & Top-5  & 0.4004 & -0.5959 & 0.1531 & 0.3799  & 0.1829 & -1.8801  & 0.1068 & 0.1735 & 0.3603 & -0.8313 & 0.1349 & 0.3427 & 0.0744 & -2.5187  & 0.0487 & 0.0699 \\
     & Top-10  & 0.3763 & -1.3345 & 0.1952 & 0.3584  & 0.1829 & -3.1084  & 0.1270 & 0.1816 & 0.3391 & -1.6383 & 0.1741 & 0.3237 & 0.0783 & -3.9772  & 0.0552 & 0.0803 \\
     & Top-20  & 0.3734 & -2.8186 & 0.2180 & 0.3793  & 0.1999 & -5.1979  & 0.1303 & 0.2244 & 0.3379 & -3.1805 & 0.1988 & 0.3449 & 0.0898 & -6.3212  & 0.0543 & 0.1077 \\
     LightGCN & Top-50  & 0.3997 & -7.1674 & 0.2068 & 0.4673  & 0.2354 & -10.5738 & 0.1037 & 0.3174 & 0.3687 & -7.5533 & 0.1951 & 0.4396 & 0.1117 & -11.9466 & 0.0449 & 0.1663 \\
    \cmidrule{2-18}
     & Rand  & 0.3875 & -3.5835 & 0.2001 & 0.4062  & 0.2075 & -6.0557  & 0.1182 & 0.2450 & 0.3527 & -3.9406 & 0.1839 & 0.3735 & 0.0938 & -7.1826  & 0.0497 & 0.1187 \\
     & Val-$k$  & 0.4652 & 0.0417  & 0.2225 & 0.4894  & 0.2296 & -0.4288  & 0.1286 & 0.2620 & 0.4253 & -0.0864  & 0.1953 & 0.4439 & 0.1017 & -0.8469  & 0.0532 & 0.1247 \\
    \cmidrule{2-18}
     & AttnCut  & 0.4749 & -0.0412 & 0.2237 & 0.4899  & 0.2260 & -0.5616  & 0.1291 & 0.3186 & 0.4242 & -0.1527 & 0.2041 & 0.4359 & 0.1121 & -0.8162  & 0.0516 & 0.1707 \\
     & MtCut  & 0.4761 & 0.1171  & 0.2318 & 0.4949  & 0.2369 & -0.5487  & 0.1319 & 0.3223 & 0.4317 & 0.0649 & 0.2113 & 0.4440 & 0.1185 & -0.8162  & 0.0536 & 0.1761 \\
     \cmidrule{2-18}
     & PerK  & \textbf{0.4993} & \textbf{0.3309}  & \textbf{0.2489} & \textbf{0.5702}  & \textbf{0.2551} & \textbf{-0.3989}  & \textbf{0.1383} & \textbf{0.3438} & \textbf{0.4543} & \textbf{0.0876}  & \textbf{0.2277} & \textbf{0.4742} & \textbf{0.1261} & \textbf{-0.7912}  & \textbf{0.0571} & \textbf{0.1878} \\
     & \textit{Improv.} & 4.87\%* &    -     & 7.38\%* & 15.22\%* & 7.68\%* &   -       & 4.85\%* & 6.67\%* & 5.24\%* &    -     & 7.76\%* & 6.80\%* & 6.41\%* &    -      & 6.53\%* & 6.64\%* \\
    \bottomrule
  \end{tabular}}
\end{sidewaystable} %\end{table*}
